Transferring Inductive Biases through Knowledge Distillation

Having the right inductive biases can be crucial in many tasks or scenarios where data or computing resources are a limiting factor, or where training data is not perfectly representative of the conditions at test time. However, defining, designing and efficiently adapting inductive biases is not necessarily straightforward. In this paper, we explore the power of knowledge distillation for transferring the effect of inductive biases from one model to another. We consider families of models with different inductive biases, LSTMs vs. Transformers and CNNs vs. MLPs, in the context of tasks and scenarios where having the right inductive biases is critical. We study the effect of inductive biases on the solutions the models converge to and investigate how and to what extent the effect of inductive biases is transferred through knowledge distillation, in terms of not only performance but also different aspects of converged solutions.

==> figs/cl_calibration.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{images/cl_lstm_v11_calibrarion.png}
    \caption{Independent LSTM
    \label{fig:cl_calibration_lstm}}
    \end{subfigure}%
     \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{images/cl_bertv10_calibrarion.png}
    \caption{Independent \transformer
    \label{fig:cl_calibration_bert}}
    \end{subfigure}%
     \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{images/cl_bert_L11toB_calibrarion.png}
    \caption{LSTM -> \transformer
    \label{fig:cl_calibration_l2b}}
    \end{subfigure}
    \caption{Calibration plots for independent and distilled Transformer for the classification setup. Green bars show perfect calibration. 
    \label{fig:cl_calibration}}
\end{figure*}

==> tex_tables/baselines_lm.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{  l  c | c  c  c  }
        \hline
        \multicolumn{2}{c}{\textbf{Model}} & \textbf{Test Perplexity\downarrow} & \textbf{Macro Accuracy(Att)\uparrow} & \textbf{Macro Accuracy(Dist)\uparrow} \\ \hline
        \textbf{Big LSTM} & exp & 56.9391 $\pm$ 0.0874 &  0.9320 $\pm$ 0.00018 & 0.9477 $\pm$ 0.0008  \\ 
        & crs & 56.1461 $\pm$ 0.0906& \textbf{0.9400} $\pm$ 0.0034& \textbf{0.9501} $\pm$ 0.0018\\ \\
        \textbf{LSTM}  & exp & 58.4136	$\pm$ \textbf{0.0254} & 0.9327 $\pm$ 0.0029 & 0.9472 $\pm$  0.0011 \\
        & crs & 59.0453 $\pm$	0.1341 & 0.9366 $\pm$ 0.0015 &	0.9491 $\pm$ 0.0010\\ \\
        \textbf{Big Transformer} & exp &  57.4977	$\pm$ 0.1199 & 0.9191 $\pm$	0.0018 & 0.9417 $\pm$ 0.0017  \\
        & crs & 61.6199 $\pm$ 0.2082 & \textbf{0.9053} $\pm$ 0.0053 & \textbf{0.9399} $\pm$ 0.0017\\ \\
        \textbf{Transformer} &  exp & 55.5117	$\pm$ 0.0607 & 0.9258 $\pm$	0.0047 & 0.9455 $\pm$ 0.0007\\ 
        % 		
        & crs & \textbf{55.3256} $\pm$ 0.0847 & 0.9261 $\pm$ 0.0020 & 0.9467 $\pm$ 0.0012\\\hline
    \end{tabular}
    \caption{Performance of the models trained on LM objective independently (mean$\pm$std over multiple trials).
     \label{tab:baselines_lm}
    }
   
\end{table*}


%bl v1
%56.9391	& 0.9320	0.9477
%0.0874	    0.0018	0.0008

%bl v10
% 56.5240	0.9329	0.9483
% 0.9100	0.0045	0.0017

%bl v20
% 56.1461	0.9400	0.9501
% 0.0906	0.0034	0.0018

%sl v1
% 58.4136	0.9327	0.9472
% 0.0254	0.0029	0.0011

%sl v10
% 58.8173	0.9312	0.9474
% 0.1207	0.0029	0.0024

%sl v20
% 59.0453	0.9366	0.9491
% 0.1341	0.0015	0.0010

%bt v1
% 57.4977	0.9191	0.9417
% 0.1199	0.0018	0.0017

%bt v10
% 57.4596	0.9136	0.9399
% 0.2372	0.0038	0.0024

%bt v20
% 61.6199	0.9053	0.9399
% 0.2082	0.0053	0.0017

%st v1
% 55.5117	0.9258	0.9455
% 0.0607	0.0047	0.0007

%st v10
% 55.7753	0.9241	0.9453
% 0.2237	0.0056	0.0027

%st v20
% 55.3256	0.9261	0.9467
% 0.0847	0.0020	0.0012



==> tex_tables/distill6_lm.tex <==
\begin{table}[]
    \centering
    \begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{c|c|c}
         \textbf{Teacher} & \textbf{Perplexity} & \textbf{Macro Accuracy(Att)}  \\ \hline
         \textbf{LSTM} & 57.7086 $\pm$ 0.0202 & 0.9333 $\pm$ 0.0015\\
         \textbf{Big LSTM} & &\\ 
    \end{tabular}
    \end{adjustbox}
    \caption{Mixed distillation results for big Transformer when the objective function is language modelling.}
    \label{tab:distill6_lm}
\end{table}

\begin{table}[]
    \centering
    \begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{l|c|c}
         \textbf{Student} & \textbf{Accuracy} $\uparrow$& \textbf{Macro Accuracy(Att)} $\uparrow$ \\ \hline
         \textbf{LSTM} & 57.7086 $\pm$ 0.0202 & 0.9333 $\pm$ 0.0015\\
         \textbf{Universal Transformer} & &\\ 
         \textbf{Transformer Decoder} & &\\ 
         \textbf{Transformer Encoder} & &\\ 
    \end{tabular}
    \end{adjustbox}
    \caption{Mixed distillation results for LSTM teacher when the objective function is classification (mean$\pm$std over multiple trials).}
    \label{tab:distill6_lm}
\end{table}

==> tex_tables/hparams.tex <==

\begin{table}[]
    \centering
    \begin{adjustbox}{width=\textwidth}
    
    
    \begin{tabular}{l | c | c | c | c   }
         model & arch. details & num. trainable params & regularization & init. learning rate  \\ \hline
         \multicolumn{5}{c}{Verb Number Classification} \\ \hline
         \transformer & d=6, h=128, num. heads=8 & & inp. drop= , h drop=, l2=, l1= & 0.0001 \\
         \seqtransformer & d=6, h=128, num. heads=8 & & inp. drop= , h drop=, l2=, l1= & 0.0001\\
         \sequniversaltransformer &  d=6, h=128, num. heads=8 & & inp. drop= , h drop=, l2=, l1= & 0.0001\\
         LSTM &  d=2, h=256 &  & inp. drop= , h drop=, l2=, l1= & 0.0001\\ \hline
         
         \multicolumn{5}{c}{Language Modelling}\\ \hline
         LSTM & d=2, h=1024 &  & inp. drop= , h drop=, l2=, l1= & 0.0001\\
         Small LSTM & d=2, h=512 &  & inp. drop= , h drop=, l2=, l1= & 0.0001  \\
         Transformer & d=6, h=512, num. heads=8 &  & inp. drop= , h drop=, l2=, l1= & 0.0001\\
         Small Transformer & d=6, h=256, num. heads=8 &  & inp. drop= , h drop=, l2=, l1= & 0.0001 \\ \hline
         
         \multicolumn{5}{c}{Digit Classification}\\ \hline
         CNN & d=3, filters=(128, 64, 64), kernels=(3, 3, 3), pool size = (1, 2, 2), &  & inp. drop=0 , h drop=0.3, l2=0.00001 & 0.0001\\
         MLP & d=3, h=(512, 128, 32) &  & inp. drop=0 , h drop=0.1, l2=0.00001, l1=0.00001 & 0.0001\\ \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Caption}
    \label{tab:hparams}
\end{table}

==> tex_tables/lm_full_baselines.tex <==
\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=0.75\textwidth}
    \begin{tabular}{  l | c  c  c  }
        \toprule
        \textbf{Model} & \textbf{Perplexity} $\downarrow$  & \textbf{\daccuracy} $\uparrow$ & \textbf{\aaccuracy} $\uparrow$\\ \midrule
          \textbf{Transformer} \\ 
        \textbf{Small Transformer} &\\
        \textbf{LSTM} &\\ 
        \textbf{Small LSTM} &  \\ 
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Performance (mean$\pm$std over multiple trials) of different LSTM and Transformer models trained independently with the LM objective on the train set.
     \label{tab:baselines_lm}
    }
% \vspace{-10pt}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=0.75\textwidth}
    \begin{tabular}{  l | c  c  c  }
        \toprule
        \textbf{Model} & \textbf{Perplexity} $\downarrow$  & \textbf{\daccuracy} $\uparrow$ & \textbf{\aaccuracy} $\uparrow$\\ \midrule
          \textbf{Transformer} \\ 
        \textbf{Small Transformer} &\\
        \textbf{LSTM} &\\ 
        \textbf{Small LSTM} &  \\ 
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Performance (mean$\pm$std over multiple trials) of different LSTM and Transformer models trained independently with the LM objective on the validation set.
     \label{tab:baselines_lm}
    }
% \vspace{-10pt}
\end{table*}

==> tex_tables/online_dstl.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Online distillation results for language modelling}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Online distillation results for classification (mean$\pm$std over multiple trials).}
    \label{tab:my_label}
\end{table}
